Interpreting Answers to Yes-No Questions in User-Generated Content

Interpreting answers to yes-no questions in social media is difficult. Yes and no keywords are uncommon, and the few answers that include them are rarely to be interpreted what the keywords suggest. In this paper, we present a new corpus of 4,442 yes-no question-answer pairs from Twitter. We discuss linguistic characteristics of answers whose interpretation is yes or no, as well as answers whose interpretation is unknown. We show that large language models are far from solving this problem, even after fine-tuning and blending other corpora for the same problem but outside social media.

==> figures/first_instance.tex <==
\begin{figure}
\graphicspath{ {./figures/images} }
\includegraphics[width=\columnwidth]{first_instance_enhanced_3.png}
\caption{
	Yes-No question from Twitter and three answers.
	Interpreting the answers is challenging and cannot be reduced to finding keywords for \emph{yes} or \emph{no}.
	The first answer ought to be interpreted as \emph{yes} since the author finds somebody else not doing so very strange.
	The second answer provides an alternative to preheating thus the interpretation is \emph{no}.
	The third answer provides an explanation of why the author does not preheat the oven.
}
\begin{comment}
	The first answer mentions that
	from and answer from twitter.
	Shown is a yes-no type question tweet.
	The first answer is an indirect answer.
	This answer compares an external entity's behavior
	(the answerer's girlfirend) 
	to the answerer's personal opinion. 
	The behavior of not preheating the oven is found to be strange by the author.
	We hence conclude that the answerer preheats the oven. 
	The \emph{interpretation} of the indirect answer is \emph{'Yes'}.
	The second answer states an alternate of "extra 3 minutes to cook".
	The argument is further strengthened by stating that certain type of ovens
	are decent like this anyway.
	We hence conclude that the author of the second answer does not preheat the oven.
	The interpretation of the indirect answer is \emph{'No'}.
	The third answer suggests not even turning on the oven. 
	The idea of pre-heating is not relevant here,
	since the author did not turn the oven on in the first place. 
	The interpretation of the indirect answer is \emph{'Unknown'}.
}
\end{comment}
\end{figure}

==> figures/keyword_heatmap.tex <==
\graphicspath{ {./figures/images} }
\includegraphics[width=6cm]{keyword_confusion.png}


==> tables/expt_results.tex <==
\begin{tabular}{l cccc@{}l@{\hspace{.05in}}l ccccc} %P{.30in}P{.30in}P{.30in}P{.30in}P{.30in}}
\toprule
& \multicolumn{5}{c}{Overall} && Yes & No & Pyes & Pno & Unk \\ \cmidrule(lr){2-6} \cmidrule(lr){8-12}
& Accuracy & P & R & F1 &&& F1 & F1 & F1 & F1 & F1 \\ \midrule
\multicolumn{10}{l}{Baselines} \\ \midrule
Majority Class & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
Keyword Based Rules & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
Keyword Based Rules + Negation Cue Detector & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ \midrule
\multicolumn{10}{l}{RoBERTa pretrained on relevant yes/no question corpora} \\ \midrule
BoolQ & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Circa & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
SwDA-IA & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Friends-QIA & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Tennis + Movie & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
Twitter-YN (Question only) & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
Twitter-YN (Answer only) & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
Twitter-YN (Question + Answer) & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ \midrule
\multicolumn{10}{l}{RoBERTa on blending Twitter-YN with relevant yes/no question corpora } \\ \midrule
BoolQ & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Circa & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
SWDA-IA & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Friends-QIA & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
Tennis + Movie & 0.00 & 0.00 & 0.00 & 0.00 &&& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\bottomrule

\end{tabular}

==> tables/gpt3_results.tex <==
\begin{tabular}{l cccc@{}l@{\hspace{.05in}}l ccccc} %P{.30in}P{.30in}P{.30in}P{.30in}P{.30in}}
\toprule
& \multicolumn{5}{c}{All} && Yes & No & Pyes & Pno & Unk \\ \cmidrule(lr){2-6} \cmidrule(lr){8-12}
& Accuracy & P & R & F1 &&& F1 & F1 & F1 & F1 & F1 \\ \midrule

% \multicolumn{10}{l}{RoBERTa (with our best weights)} \\
RoBERTa (best weights)
& 0.60 & 0.59 & 0.60 & 0.59 &&& 0.71 & 0.62 & 0.37 & 0.26 & 0.53 \\
~~~+Disambiguation text from GPT3
& 0.58 & 0.60 & 0.58 & 0.53 &&& 0.71 & 0.60 & 0.19 & 0.12 & 0.36 \\ 
\midrule

\multicolumn{10}{l}{GPT3} \\
~~~Zero shot
& 0.44 & 0.55 & 0.44 & 0.46 &&& 0.56 & 0.51 & 0.16 & 0.13 & 0.43 \\
~~~~~~+Annotation guidelines
& 0.42 & 0.55 & 0.42 & 0.41 &&& 0.51 & 0.48 & 0.12 & 0.00 & 0.40 \\ 

~~~Few shot
& 0.54 & 0.55 & 0.54 & 0.53 &&& 0.67 & 0.55 & 0.14 & 0.30 & 0.49 \\
~~~~~~+Annotation guidelines
& 0.52 & 0.57 & 0.52 & 0.50 &&& 0.66 & 0.50 & 0.15 & 0.16 & 0.48 \\

\bottomrule
\end{tabular}

==> tables/label_descriptions.tex <==
\begin{table}[]
\noindent\rule{8cm}{0.8pt}
Question: blah?\\
Answer: blah\\
\emph{Implicit direct answer: Yes (y)}\\
\noindent\rule{8cm}{0.4pt}
Question: blah?\\
Answer: blah.\\
\emph{Implicit direct answer: Probably Yes (py)}\\
\noindent\rule{8cm}{0.4pt}
Question: blah?\\
Answer: blah.\\
\emph{Implicit direct answer: No (n)}\\
\noindent\rule{8cm}{0.4pt}
Question: blah?\\
Answer: blah.\\
\emph{Implicit direct answer: Probably No (pn)}\\
\noindent\rule{8cm}{0.4pt}
Question: blah?\\
Answer: blah.\\
\emph{Implicit direct answer: Unknown (uk)}\\
\noindent\rule{8cm}{0.8pt}
\caption{Question and reply tweet instances in Twitter-YN.  The implicit direct answer for each question answer instance is also shown. We show an example for each of the five classes.}
\label{different_classes}
\end{table}

==> tables/label_explained.tex <==
\begin{tabular}{p{5cm}p{1cm}}
\toprule
& \multicolumn{1}{p{2cm}}{Interpretation}\\
\multicolumn{1}{p{5cm}}{Question 1: Do you think only people with a certain level of political knowledge should be allowed to vote?}\\
\\
\multicolumn{1}{p{5cm}}{Answer 1.1: effective democracy relies on an informed populace. i don't think that's where we are.}& \multicolumn{1}{c}{Yes} \\
\\
\multicolumn{1}{p{5cm}}{Answer 1.2: explain how you would judge someone's levels of know in politics, sounds very patronising to me}& \multicolumn{1}{c}{No} \\
\\
\multicolumn{1}{p{5cm}}{Answer 1.3: i don't think politics should exist.}& \multicolumn{1}{c}{Unknown} \\
\midrule
% & \multicolumn{1}{p{2cm}}{Interpretation}\\
\multicolumn{1}{p{5cm}}{Question 2: On a work zoom, is it unprofessional to obviously be in your bed?}\\
\\
\multicolumn{1}{p{5cm}}{Answer 2.1: lol! only if they can see you}& \multicolumn{1}{c}{Probably Yes} \\
\\
\multicolumn{1}{p{5cm}}{Answer 2.2: anyone who would be working with you needs to know you’re a bed boy}& \multicolumn{1}{c}{Probably No} \\
\bottomrule
\end{tabular}

==> tables/motivation_examples.tex <==
\setlength{\tabcolsep}{.02in}
\newcommand\w{2.8in}

\begin{table}[]
\noindent\rule{8cm}{0.8pt}
Question: Do you start projects you don't intend to finish?\\
Answer: i used to be able to finish any tweet but now i\\
\emph{Implicit direct answer: Yes}\\
\noindent\rule{8cm}{0.4pt}
Question: Do you like rift?\\
Answer: i meant to say yes and hit no by accident.\\
\emph{Implicit direct answer: Yes}\\
\noindent\rule{8cm}{0.8pt}
\caption{Examples showing the indirect reply tweet to a yes-no type question tweet. The implicit direct answer is also shown.  We see that indirect reply tweets can be pun related and/or can contain yes or no related token(s) that may not agree to the implicit direct answer.}
\label{intro_example}
\end{table}
